Temporal Inductive Logic Reasoning over Hypergraphs

Inductive logic reasoning is a fundamental task in graph analysis, which aims to generalize patterns from data. This task has been extensively studied for traditional graph representations, such as knowledge graphs (KGs), using techniques like inductive logic programming (ILP). Existing ILP methods assume learning from KGs with static facts and binary relations. Beyond KGs, graph structures are widely present in other applications such as procedural instructions, scene graphs, and program executions. While ILP is beneficial for these applications, applying it to those graphs is nontrivial: they are more complex than KGs, which usually involve timestamps and n-ary relations, effectively a type of hypergraph with temporal events. In this work, we propose temporal inductive logic reasoning (TILR), an ILP method that reasons on temporal hypergraphs. To enable hypergraph reasoning, we introduce the multi-start random B-walk, a novel graph traversal method for hypergraphs. By combining it with a path-consistency algorithm, TILR learns logic rules by generalizing from both temporal and relational data. To address the lack of hypergraph benchmarks, we create and release two temporal hypergraph datasets: YouCook2-HG and nuScenes-HG. Experiments on these benchmarks demonstrate that TILR achieves superior reasoning capability over various strong baselines.

==> parts/nuscence-stats-and-fig.tex <==
\begin{figure*}[t]
    \begin{minipage}{\textwidth}
    \begin{minipage}[b]{0.62\textwidth}
        \centering 
        \resizebox{\linewidth}{!}{%
        \begin{tabular}[b]{@{}llcccc@{}}
        \toprule
        \multicolumn{2}{l}{\multirow{2}{*}{Predicate Type}} & \multirow{2}{*}{\# Predicates} & \multicolumn{2}{c}{\# Facts}                     & \multirow{2}{*}{Examples} \\
        \multicolumn{2}{l}{}                                &                                & Per Graph             & Total                    &                           \\ \midrule
        \multirow{4}{*}{Relation} & \multirow{2}{*}{Unary}  & \multirow{2}{*}{13}            & \multirow{2}{*}{4631} & \multirow{2}{*}{3473257} & ego.throttle              \\
                                  &                         &                                &                       &                          & ego.brake                 \\
                                  & \multirow{2}{*}{Binary} & \multirow{2}{*}{6}             & \multirow{2}{*}{1859} & \multirow{2}{*}{1394253} & in\_front                 \\
                                  &                         &                                &                       &                          & behind                    \\
                                  & N-ary                   & 1                              & 1692                  & 1269004                  & Between                   \\ \midrule
        \multicolumn{2}{c}{\multirow{3}{*}{Class}}          & \multirow{3}{*}{23}            & \multirow{3}{*}{257}  & \multirow{3}{*}{45881}   & vehicle.car               \\
        \multicolumn{2}{c}{}                                &                                &                       &                          & human.pedestrian.adult    \\
        \multicolumn{2}{c}{}                                &                                &                       &                          & ped\_crossing             \\ \bottomrule
        \end{tabular}%
        }
        \captionof{table}{Statistics of the temporal hypergraph benchmark based on the nuScenes autonomous driving datasets.}
        \label{tab:auto-drive}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/nuscene-example.png}
        \captionof{figure}{Example driving logs in nuScenes.}
        \label{fig:nuscene-example}
    \end{minipage}
\end{minipage}
\end{figure*}

==> parts/res-table-nuscences.tex <==
\begin{table}[t]
\centering
\resizebox{0.65\linewidth}{!}{%
\begin{tabular}{@{}lrrr@{}}
\toprule
\multirow{2}{*}{Method} & \multicolumn{3}{c}{nuScenes Hypergraph} \\
 & \multicolumn{1}{c}{MRR} & \multicolumn{1}{c}{H@3} & \multicolumn{1}{c}{H@10} \\ \midrule
MRBW & 0.19 & 20.8 & 31.4 \\
MRBW+PC & 0.22 & 24.1 & 35.5 \\
MRBW+PC (train) & 0.46 & 45.3 & 52.7 \\ \bottomrule
\end{tabular}%
}
\caption{MRR and Hits of the three versions of MRBW on the nuScenes hypergraph benchmark.}
\label{tab:nuscenes-results}
\vspace{-.4cm}
\end{table}

==> parts/res-table-youcook2.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lrrrccc@{}}
\toprule
\multirow{2}{*}{Method} & \multicolumn{3}{c}{Clique-Expansion} & \multicolumn{3}{c}{Hypergraph} \\ \cmidrule(l){2-7} 
 & \multicolumn{1}{c}{MRR} & \multicolumn{1}{c}{H@3} & \multicolumn{1}{c}{H@10} & MRR & H@3 & H@10 \\ \midrule
GNN-GCN & 0.76 & 79.2 & 82.1 & - & - & - \\
GNN-Cheb & 0.78 & 80.7 & 82.9 & - & - & - \\
CTDNE & 0.81 & 85.3 & 87.6 & - & - & - \\ \midrule
RW & 0.19 & 18.8 & 20.6 & - & - & - \\
NeuralLP & 0.36 & 37.1 & 39.5 & - & - & - \\ \midrule
MRBW & 0.25 & 20.4 & 23.7 & \multicolumn{1}{r}{0.35} & \multicolumn{1}{r}{29.4} & \multicolumn{1}{r}{36.3} \\
MRBW+PC & 0.30 & 27.9 & 31.1 & \multicolumn{1}{r}{0.60} & \multicolumn{1}{r}{55.8} & \multicolumn{1}{r}{59.1} \\
MRBW+PC (train) & 0.42 & 38.2 & 42.5 & \multicolumn{1}{r}{0.72} & \multicolumn{1}{r}{76.0} & \multicolumn{1}{r}{79.4} \\ \bottomrule
\end{tabular}%
}
\caption{MRR and Hits of three MRBW methods on recipe summarization task together with that of three GNN-based methods and two static graph ILP methods.}
\label{tab:recipe-results}
\end{table}
